Quantitative Verification of Masked Arithmetic Programs against Side-Channel Attacks

Power side-channel attacks, which can deduce secret data via statistical analysis, have become a serious threat. Masking is an effective countermeasure for reducing the statistical dependence between secret data and side-channel information. However, designing masking algorithms is an error-prone process. In this paper, we propose a hybrid approach combing type inference and model-counting to verify masked arithmetic programs against side-channel attacks. The type inference allows an efficient, lightweight procedure to determine most observable variables whereas model-counting accounts for completeness. In case that the program is not perfectly masked, we also provide a method to quantify the security level of the program. We implement our methods in a tool QMVerif and evaluate it on cryptographic benchmarks. The experimental results show the effectiveness and efficiency of our approach.

==> maintech.tex <==
%\section{Inference Algorithms}
\section{Three Key Techniques}
\label{sec:3proc}
In this section, we introduce three key techniques: type inference system, SMT-based reasoning and reduction techniques, which will be used in our verification algorithm.

\input{type_system}

\input{smt-based}

\input{exprsimplify}


==> related_work.tex <==
\section{Related Work}
\label{sec:rel}
 
